The Atacama Cosmology Telescope: Constraints on Cosmic Birefringence

We present new constraints on anisotropic birefringence of the cosmic microwave background polarization using two seasons of data from the Atacama Cosmology Telescope covering $456$ square degrees of sky. The birefringence power spectrum, measured using a curved-sky quadratic estimator, is consistent with zero. Our results provide the tightest current constraint on birefringence over a range of angular scales between $5$ arcminutes and $9$ degrees. We improve previous upper limits on the amplitude of a scale-invariant birefringence power spectrum by a factor of between $2$ and $3$. Assuming a nearly-massless axion field during inflation, our result is equivalent to a $2\,\sigma$ upper limit on the Chern-Simons coupling constant between axions and photons of $g_{\alpha\gamma}<4.0\times 10^{-2}/H_I$ where $H_I$ is the inflationary Hubble scale.

==> authorlist_arXiv.tex <==
Toshiya Namikawa, Yilun Guan, Omar Darwish, Blake D. Sherwin, Simone Aiola, Nicholas Battaglia, James A. Beall, Daniel T. Becker, J. Richard Bond, Erminia Calabrese, Grace E. Chesmore, Steve K. Choi, Mark J. Devlin, Joanna Dunkley, Rolando D\"unner, Anna E. Fox, Patricio A. Gallardo, Vera Gluscevic, Dongwon Han, Matthew Hasselfield, Gene C. Hilton, Adam D. Hincks, Ren\'ee Hlo\v{z}ek, Johannes Hubmayr, Kevin Huffenberger, John P. Hughes, Brian J. Koopman, Arthur Kosowsky, Thibaut Louis, Marius Lungu, Amanda MacInnis, Mathew S. Madhavacheril, Maya Mallaby-Kay, Lo\"ic Maurin, Jeffrey McMahon, Kavilan Moodley, Sigurd Naess, Federico Nati, Laura B. Newburgh, John P. Nibarger, Michael D. Niemack, Lyman A. Page, Frank J. Qu, Naomi Robertson, Alessandro Schillaci, Neelima Sehgal, Crist\'obal Sif\'on, Sara M. Simon, David N. Spergel, Suzanne T. Staggs, Emilie R. Storer, Alexander van Engelen, Jeff van Lanen, Edward J. Wollack
